How Good MVSNets Are at Depth Fusion

We study the effects of the additional input to deep multi-view stereo methods in the form of low-quality sensor depth. We modify two state-of-the-art deep multi-view stereo methods for using with the input depth. We show that the additional input depth may improve the quality of deep multi-view stereo.

==> src/main/authors_background.tex <==
\section*{Author's background}
\centerline{
\setlength\tabcolsep{\widthof{0}*\real{.6}}
\setlength\aboverulesep{0pt}
\setlength\belowrulesep{0pt}
\begin{tabular}{|c|c|c|c|}
    \midrule
    Oleg Voynov & Phd candidate & Computer vision, 3D Deep learning & \\
    \midrule
    Aleksandr Safin & Phd candidate & Computer vision, 3D Deep learning & \\
    \midrule
    Savva Ignatyev & Phd candidate & Computer vision, 3D Deep learning & \\
    \midrule
    Evgeny Burnaev & Associate professor & \makecell{Kernel methods, Surrogate modeling,\\Anomaly detection, Online learning,\\3D/4D Deep learning} & \href{https://faculty.skoltech.ru/people/evgenyburnaev}{faculty.skoltech.ru/people/evgenyburnaev} \\
    \midrule
\end{tabular}
}

